Verification of Building Blocks for Asynchronous Circuits

Scalable formal verification constitutes an important challenge for the design of asynchronous circuits. Deadlock freedom is a property that is desired but hard to verify. It is an emergent property that has to be verified monolithically. We present our approach to using ACL2 to verify necessary and sufficient conditions over asynchronous delay-insensitive primitives. These conditions are used to derive SAT/SMT instances from circuits built out of these primitives. These SAT/SMT instances help in establishing absence of deadlocks. Our verification effort consists of building an executable checker in the ACL2 logic tailored for our purpose. We prove that this checker is correct. This approach enables us to prove ACL2 theorems involving defun-sk constructs and free variables fully automatically.

==> eptcsdata.tex <==
\providecommand{\firstpage}{70}
\providecommand{\publicationstatus}{R. Gamboa and J. Davis (Eds.): ACL2 Workshop 2013 (ACL2 '13).\\
EPTCS 114, 2013, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.114.6}{10.4204/EPTCS.114.6}}

